Data-driven joint optimization of maintenance and spare parts provisioning: A distributionally robust approach

This paper investigates the joint optimization of condition-based maintenance and spare provisioning, incorporating insights obtained from sensor data. Prognostic models estimate components' remaining lifetime distributions (RLDs), which are integrated into an optimization model to coordinate maintenance and spare provisioning. The existing literature addressing this problem assumes that prognostic models provide accurate estimates of RLDs, thereby allowing a direct adoption of Stochastic Programming or Markov Decision Process methodologies. Nevertheless, this assumption often does not hold in practice since the estimated distributions can be inaccurate due to noisy sensors or scarcity of training data. To tackle this issue, we develop a Distributionally Robust Chance Constrained (DRCC) formulation considering general discrepancy-based ambiguity sets that capture potential distribution perturbations of the estimated RLDs. The proposed formulation admits a Mixed-Integer Linear Programming (MILP) reformulation, where explicit formulas are provided to simplify the general discrepancy-based ambiguity sets. Finally, for the numerical illustration, we test a type-$\infty$ Wasserstein ambiguity set and derive closed-form expressions for the parameters of the MILP reformulation. The efficacy of our methodology is showcased in a wind turbine case study, where the proposed DRCC formulation outperforms other benchmarks based on stochastic programming and robust optimization.

==> sections/P0_abstract.tex <==
{\normalsize \textbf{Abstract. } } \textbf{Problem definition:} This paper investigates the joint optimization of condition-based maintenance and spare provisioning, incorporating insights obtained from sensor data. Predictive analytics models estimate components' remaining lifetime uncertainty. The estimated distributions are integrated into an optimization to coordinate maintenance and spare provisioning. The existing literature addressing this problem assumes that predictive analytics models provide an accurate estimate of the uncertainty, thereby allowing the direct implementation of Stochastic Programming or Markov Decision Process methodologies. Nevertheless, this assumption often does not hold in practice because the estimated distributions can be biased due to noisy sensors or sparsity in training data. \textbf{Methodology/results:} Our decision model acknowledges that the estimated distributions can be inaccurate and so seeks optimal solutions that are robust against distribution perturbations. We develop a Distributionally Robust Chance Constrained (DRCC) formulation, which uses the estimated distributions as a reference to construct a Wasserstein ambiguity set that captures potential distribution perturbations. We demonstrate that the proposed DRCC optimization problem admits an exact mixed integer linear programming reformulation that can be efficiently solved by off-the-shelf optimizer software. The efficacy of our methodology is showcased in a case study on wind turbines, where the proposed DRCC formulation outperforms other benchmark models based on stochastic programming and robust optimization, especially when dealing with inaccurate predictive analytics results. 
\textbf{Managerial implications:} The proposed joint optimization formulation enables the seamless coordination between maintenance schedule and spare provisioning, even when dealing with inaccurate predictive analytics results. The formulation incorporates insights obtained from real-time sensor data robustly, thus adapting maintenance and spare management decisions to the degradation experienced by the physical components. As a consequence, our model can mitigate the risk of unexpected failures without incurring conservative
maintenance policies.

==> sections/P2_Literature_review.tex <==
\section{Literature Review} \label{sec:literature_review}

The optimization of maintenance schedules and spare inventory for industrial components has been traditionally studied separately. Maintenance models assume that spare parts are always available in stock, and so make decisions based solely on lifetime or remaining lifetime distributions \citep{barlow1960optimum,jardine1997optimal,drent2023real,yildirim2016sensor}. Spare inventory models, on the other hand, usually rely on time-series methodologies to predict the demand for spare parts based on the historical spare demand without considering the impact of maintenance decisions \citep{li2011bayesian,van2019forecasting,howard2015inventory}. Nevertheless, optimizing these two problems in isolation or a sequential fashion can lead to sub-optimal solutions due to the tight coupling between spare inventory and maintenance decisions \citep{van2013joint}. The above has motivated the development of new methodologies to optimize maintenance schedules and spare provisioning jointly. 


The joint optimization of maintenance and spare provisioning have been investigated under varied approaches. A thorough survey on this topic is presented in \citep{van2013joint}. The first papers on this topic focused on threshold-based policies using reliability distributions. For example, \cite{kabir1996stocking} developed a joint policy, known as the (s, S, t) stocking policy, which minimizes the long-run total cost of replacement and spare parts inventory. In this policy, the reorder point is denoted by $s$, the order-up-to level is denoted by $S$, and a specified age for preventive maintenance is denoted by $t$. The optimal policy was obtained through simulation. This work was extended in \citep{sarker2000optimization} by incorporating additional factors, such as different costs associated with different inventory levels, the number of failures, and the placement of emergency orders when the inventory level falls abruptly. \cite{hu2008joint} also extended this model by implementing a genetic algorithm to reduce the objective value and the running time. A notable limitation of this line of work is that the models rely on reliability information instead of CM data. This can lead to conservative policies that usually recommend frequent, unnecessary repairs to protect against unexpected failures \citep{yildirim2016sensor}.



The widespread adoption of Internet of Things (IoT) technologies has boosted the implementation of CBM strategies in industrial applications \citep{olsen2020industry}. As a result, recent papers have investigated using CM strategies to jointly optimize maintenance and spare inventory \citep{rausch2010joint,
zhang2017joint, keizer2017joint,feng2023managing}. \cite{rausch2010joint} analyzed a single-unit system with a spare part inventory pool and applied bi-objective optimization to minimize the spare part inventory and the expected total operating cost. \cite{zhang2017joint} and \cite{keizer2017joint} studied a system with multiple identical units by stochastic decision processes. They developed condition-based policies for maintenance and spare provisioning relying on genetic algorithms \citep{zhang2017joint} and Markov Decision Process (MDP) \citep{keizer2017joint}. \cite{feng2023managing} investigated the joint optimization of production, inventory, and maintenance for a group of identical machines by continuous-time MDP. These models \citep{zhang2017joint, keizer2017joint,rausch2010joint,feng2023managing} generate control policies that trigger maintenance activities when a degradation signal reaches a certain threshold. However, such decisions are based solely on the current condition of the component without considering predictions of the evolution of components' degradation. Predicting components' remaining lifetime can be critical for planning future repair activities, and thus play a key role in the joint optimization problem.


Failure prognostic algorithms enable the estimation of components' RLDs based on CM data. The development of such algorithms has been prominent during the last decades--\cite{elattar2016prognostics} presents a survey on this topic. Estimated RLDs can provide advanced knowledge to jointly optimize maintenance activities and spare parts provisioning. However, the use of prognostics for jointly optimizing maintenance and spare inventory has not been studied extensively. The existing works on solving the joint optimization problem using prognostic results can be classified depending on the size of the system under study, resulting in single-unit and multi-unit system approaches. Single-unit system approaches \citep{elwany2008sensor,wang2015prognostics} deal with a system composed of a single component. Implementing these methodologies in industrial applications is limited as real-world systems often have multiple components. Multi-unit system approaches \citep{dieterman2019joint, zheng2021joint, shi2022stochastic}, on the other hand, analyze systems with multiple components. However, the existing multi-unit approaches are focused on systems with multiple \textit{identical} components. In this context, the joint optimization problem has been formulated and solved using different methodologies, including threshold-based policies \citep{dieterman2019joint}, MDP \citep{zheng2021joint}, and stochastic programming \citep{shi2022stochastic}. The existing joint optimization models using prognostic results for multi-unit systems have two main limitations. 1) They assume that the RLDs estimated by the prognostic algorithms accurately characterize the uncertainty of the components' failure times. This assumption enables the direct integration of the estimated RLDs into standard stochastic optimization frameworks, including MDPs and stochastic programming. Nevertheless, estimated RDLs can be biased due to multiple factors, such as noisy sensors or sparsity of training data. When this happens, the decisions computed using  MDPs or stochastic programming can be far from optimal because the model uncertainty differs from the real-world uncertainty. 2) They deal with multiple identical components, thus needing just one spare inventory. However, most industrial systems have multiple \textit{non-identical} components, so they need to manage multiple spare inventories accounting for the diversity of spare parts and their potential dependencies. These two critical open issues are investigated throughout this paper.


{\color{red} Summary of Contributions: Please fill in here}

==> sections/ancknowledgment.tex <==
\section*{Acknowledgment}

This work has been partially supported by FONDECYT Chile Grant No. 1210031; the Advanced Center for Electrical and Electronic Engineering, AC3E, Basal Project FB0008, ANID; and CONICYT PIA/BASAL AFB180003. Additionally, the work of Heraldo Rozas and Diego Muñoz-Carpintero has been supported by CONICYT-PFCHA/MagisterNacional/2018-22180232 and CONICYT - FONDECYT Postdoctorado - 3170040, respectively. Finally, the authors would like to thank Prof. Fernando Ordoñez (Department of Industrial Engineering, University of Chile) for kindly sharing with us average traffic speed data from an actual location in Chile.
 
 

==> sections/biblio.tex <==
\section*{Bibliography}

\addcontentsline{toc}{chapter}{\protect\numberline{}Bibliography}
%\bibliographystyle{plain}


\renewcommand{\chapter}[2]{}% for other classes
\printbibliography
